Tropical cyclones on tidally locked rocky planets: Dependence on rotation period

Tropical cyclones occur over the Earth's tropical oceans, with characteristic genesis regions and tracks tied to the warm ocean surface that provides energy to sustain these storms. The study of tropical cyclogenesis and evolution on Earth has led to the development of environmental favorability metrics that predict the strength of potential storms from the local background climate state. Simulations of the gamut of transiting terrestrial exoplanets orbiting late-type stars may offer a test of this Earth-based understanding of tropical cyclogenesis. Previous work has demonstrated that tropical cyclones are likely to form on tidally locked terrestrial exoplanets with intermediate rotation periods of $\sim 8-10~\mathrm{days}$. In this study, we test these expectations using ExoCAM simulations with both a sufficient horizontal resolution of 0.47$^\circ$ x 0.63$^\circ$ required to permit tropical cyclogenesis along with a thermodynamically active slab ocean. We conduct simulations of tidally locked and ocean-covered Earth-sized planets orbiting late-type M dwarf stars with varying rotation periods from 4-16 days in order to cross the predicted maximum in tropical cyclogenesis. We track tropical cyclones that form in each simulation and assess their location of maximum wind, evolution, and maximum wind speeds. We compare the resulting tropical cyclone locations and strengths to predictions based on environmental favorability metrics, finding good agreement between the Earth-based metrics and our simulated storms with a local maximum in both tropical cyclone frequency and intensity at a rotation period of 8 days. Our results suggest that environmental favorability metrics used for tropical cyclones on Earth may also be applicable to temperate tidally locked Earth-sized rocky exoplanets with abundant surface liquid water.

==> referee_response.tex <==

\underline{\bf Response to Comments} 
\begin{enumerate}
\item \textit{ } \\
\noindent Thank you for    \\

\underline{Line } 
\begin{quotation}
{\bf }
\end{quotation}

\end{enumerate}

